The 5 Electron Case of Thomson's Problem

We give a rigorous computer-assisted proof that the triangular bi-pyramid is the unique configuration of 5 points on the 2-sphere that globally minimizes the Coulomb (1/r) potential. We also prove the same result for the (1/r^2) potential. The main mathematical contribution of the paper is a fairly efficient energy estimate that works for any number of points and any power-law potential.

==> 3overview.tex <==

\section{Overview of the Proof}

\subsection{The Energy of the TBP}

Let $E_e$ denote the $1/r^e$ power law.
In the TBP, one pair of points is $2$ units apart,
$3$ pairs of points are $\sqrt 3$ units apart,
and $6$ pairs of points are $\sqrt 2$ units apart.
Accordingly, the energy of the TBP, with respect to $E_e$, is
\begin{equation}
\label{penta}
M_e = \frac{1}{2^e} + \frac{3}{3^{e/2}} + \frac{6}{2^{e/2}}.
\end{equation}

We call a configuration $P$ of $5$ points on $S^2$ a {\it minimizer\/} if
$E_e(P) \leq M_e$.   Our goal is to prove that $P$ is a minimizer for $e=1,2$
if and only if $P$ is the TPB.   Here we prove a crude estimate about
minimizers.    We hope that the reader will forgive the sketchiness of
our proof.  We only care about the cases $e=1$ and $e=2$ in this paper,
and in these cases we just make a direct calculation.

\begin{lemma}
Suppose $P$ is a minimizer with respect to $E_e$.
Then the minimum distance between
pairs of points in $P$ is at least $1/2$.
\end{lemma}

\startproof
The regular tetrahedron minimizes the
energy for $4$ points.    The distance between pairs of points in the
regular tetrahedron is $t=\sqrt{8/3}$.   Hence, the energy of the
regular tetrahedron is $6/t^e$.

 Letting
$P=\{p_0,...,p_4\}$, suppose that $\|p_0-p_4\| \leq 1/2$. 
Since all the points are on $S^2$, we have $\|p_0-p_i\| \leq 2$ for $i=1,2,3$.
Finally, the total energy of the points $\{p_1,p_2,p_3,p_4\}$ is at least as much as
the energy of the regular tetrahedron.
Therefore
\begin{equation}
\label{tetra}
E_e(P) \geq R_e:=2^e + \frac{3}{2^e}+ \frac{6}{t^e}=2^e + \frac{3}{2^e}+ 6\frac{3^{e/2}}{8^{e/2}}.
\end{equation}
Let $f(e)=R_e-M_e$.  A direct calculation shows that $f(1)>0$ and $f(2)>0$.

For the general case, we
calculate that $f(0)=0$ and $f'(0)>0$ and $f''(0)>1$.
An easy argument shows that $|f'''|<30$ on $[0,1/10]$.
Taylor's theorem with remainder then shows that $f>0$ on $[0,1/10]$.
A rather trivial argument shows that $f>0$ on $[4,\infty)$.   The
$2^e$ term dominates in this range.  One can show easily that
$|f'|<100$ on $[1/10,4]$.   We then check numerically that
$f(k/100)>1/100$ for $k=10,...,400$.  This fact, together with 
the bound on $|f'|$, shows that $f>0$ on $[1/10,4]$.
\endproof

\end{document}
\subsection{Stereographic Projection}

We find it convenient to work mainly with
$\C \cup \infty$ rather than on $S^2$.    
Our reason for this is that a configuration space
based on points in $\C$ has a
natural flat structure, and lends itself well
to a nice subdivision scheme.   The subdivision
scheme, which essentially amounts to cutting
rectangular solids into smaller rectangular
solids, feeds into our divide-and-conquer
algorithm.

We map $S^2$ to $\C \cup \infty$ using
{\it stereographic projection\/}:
\begin{equation}
\label{stereo}
\Sigma(x,y,z)=\frac{x}{1-z}+ i\ \frac{y}{1-z}.
\end{equation}
$\Sigma$ is a conformal diffeomorphism which maps
circles on $S^2$ to generalized circles in $\C \cup \infty$.
A {\it generalized circle\/} is either a circle or a straight line.
We have $\Sigma(0,0,1)=\infty$.   Thus, $\Sigma$ maps
a circle $C \subset S^2$ to a straight line if and only if
$(0,0,1) \in C$.

The inverse map is given by
\begin{equation}
\Sigma^{-1}(x+iy)=\bigg(\frac{2x}{1+x^2+y^2},\frac{2y}{1+x^2+y^2},
1-\frac{2}{1+x^2+y^2}\bigg).
\end{equation}

Let $\|\cdot\|$ denote the usual norm on $\R^3$.
Here are two pieces of metric information we will use later on:
\begin{equation}
\label{metric1}
\|\Sigma^{-1}(z)-\Sigma^{-1}(\infty)\|=\frac{2}{\sqrt{1+|z|^2}}
\end{equation}

\begin{equation}
\label{metric2}
\bigg{\|} \frac{d\Sigma^{-1}}{dx}\bigg{\|} =
\bigg{\|} \frac{d\Sigma^{-1}}{dy}\bigg{\|} =
\frac{2}{1+x^2+y^2}.
\end{equation} 

Equations \ref{metric1} and \ref{metric2} both have
straightforward derivations, which we omit.

Let $E$ be one of the power law energy potentials on $S^2$.
Slightly abusing notation, we define
\begin{equation}
E(z_1,z_2)=E\big(\Sigma^{-1}(z_1),\Sigma^{-1}(z_2)\big)
\end{equation}
for points $z_1,z_2 \in \C \cup \infty$.  In this way, we
can talk about the energy of a configuration of points in $\C \cup \infty$.

\subsection{Normalizing the Configuration}

Let $P=\{p_0,...,p_4\}$ be a configuration of $5$ points on $S^2$.
We let \begin{equation}
Q=\Sigma(P)=\{q_0,...,q_4\}
\end{equation}
be the corresponding
configuration on $\C \cup \infty$.  We rotate $S^2$ so that
\begin{itemize}
\item $q_4=\infty$.
\item $q_0 \in \R^+$.
\item $E(q_0,q_4) \geq E(q_i,q_j)$ for any other indices $i \not = j$.
\end{itemize}

Now we discuss what the configuration $Q$ looks like when it is
the stereographic image of the TBP.
The TBP has two kinds of points.   We say that the
{\it polar points\/} are the two antipodal points in the configuration.
We say that the three remaining points are {\it equitorial\/}.
When $q_0$ corresponds to a polar point, we have the following
configuration, which is unique up to the permutation of $q_1,q_2,q_3$:
\begin{itemize}
\item $q_0=1$.
\item $q_1=0$;
\item $q_2=\exp(2 \pi i/3)$, the usual third root of unity.
\item $q_3=\exp(4 \pi i/3)$, the other third root of unity.
\end{itemize}








\end{document}


\subsection{Patch Functions}

definition of a patch function.  main estimate.

\subsection{The Square Estimate}


\subsection{The Algorithm}

\subsection{Results about the Hessian}

\subsection{Putting it Together}

\newpage

